Constructing Printable Surfaces with View-Dependent Appearance

We present a method for the digital fabrication of surfaces whose appearance varies based on viewing direction. The surfaces are constructed from a mesh of bars arranged in a self-occluding colored heightfield that creates the desired view-dependent effects. At the heart of our method is a novel and simple differentiable rendering algorithm specifically designed to render colored 3D heightfields and enable efficient calculation of the gradient of appearance with respect to heights and colors. This algorithm forms the basis of a coarse-to-fine ML-based optimization process that adjusts the heights and colors of the strips to minimize the loss between the desired and real surface appearance from each viewpoint, deriving meshes that can then be fabricated using a 3D printer. Using our method, we demonstrate both synthetic and real-world fabricated results with view-dependent appearance.

==> 10_figonly.tex <==
\newpage

\begin{figure*}
  \centering
  \vspace*{0.05in}
  \includegraphics[scale = 0.8]{fig/siggraph.png}
  \caption{Top: Optimized surface with five distinct desired appearances. Bottom: Optimized surface with four distinct desired views.}
  \Description{}
  \label{fig:siggraph}
  \vspace*{0.1in}
\end{figure*}

\begin{figure*}
  \centering
  \vspace*{0.05in}
  \includegraphics[width=\linewidth]{fig/lenticular.png}
  \caption{Top: desired appearances. Middle: Renders of lenticular surface from three different viewing directions. Bottom: Render of self-occluding surface generated via our method from three different viewing directions.}
  \Description{}
  \label{fig:lens}
\end{figure*}


\begin{figure*}
  \centering
  \vspace*{0.05in}
  \includegraphics[width=\linewidth]{fig/physresults.png}
  \caption{Photographs of various fabricated surfaces. Top row: The same surface as viewed from four directions, displaying four unrelated colorful patterns. Bottom row: The same surface as viewed from two directions, displaying the Stanford Dragon and the Stanford Bunny.}  
  \Description{}
  \label{fig:phys}
  \vspace*{0.1in}
\end{figure*}

\begin{figure*}
    \captionsetup[subfigure]{labelformat=empty}

    \centering
    \begin{subfigure}[t]{0.45\textwidth}

        \centering
        \includegraphics[width=\linewidth]{fig/azimuthcompatibility.png} 
        \caption{Fig. 13a. MSE loss after 100 steps with two viewing directions. The first viewing direction has a desired appearance of solid black, with elevation 60 and azimuth 0. The second viewing direction has a desired appearance of solid white, elevation 60 degrees and variable azimuth.} \label{fig:azimuth}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}

        \centering
        \includegraphics[width=\linewidth]{fig/elevationcompatibility.png} 
        \caption{Fig. 13b. MSE loss after 100 steps with two viewing directions. The first viewing direction has a desired appearance of solid black, with elevation 20 and azimuth 0. The second viewing direction has a desired appearance of solid white, variable elevation and azimuth 0.} \label{fig:elevation}
    \end{subfigure}

\end{figure*}




\begin{figure*}
    \captionsetup[subfigure]{labelformat=empty}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[scale = 0.2]{fig/checks.png} 
        \caption{Fig. 14a. Top: Render of synthetic surface as viewed from two directions. Bottom: Fabricated version of this same surface.} \label{fig:simtoreal}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{fig/bike.png} 
        \caption{Fig. 14b. High-resolution fabrication of a biking/no biking sign as viewed from two high-elevation directions  (60 degrees). The surface is less than 1cm wide.} \label{fig:bike}
    \end{subfigure}
\end{figure*}






